A Comparative Study of Brain Reproduction Methods for Morphologically Evolving Robots

In the most extensive robot evolution systems, both the bodies and the brains of the robots undergo evolution and the brains of 'infant' robots are also optimized by a learning process immediately after 'birth'. This paper is concerned with the brain evolution mechanism in such a system. In particular, we compare four options obtained by combining asexual or sexual brain reproduction with Darwinian or Lamarckian evolution mechanisms. We conduct experiments in simulation with a system of evolvable modular robots on two different tasks. The results show that sexual reproduction of the robots' brains is preferable in the Darwinian framework, but the effect is the opposite in the Lamarckian system (both using the same infant learning method). Our experiments suggest that the overall best option is asexual reproduction combined with the Lamarckian framework, as it obtains better robots in terms of fitness than the other three. Considering the evolved morphologies, the different brain reproduction methods do not lead to differences. This result indicates that the morphology of the robot is mainly determined by the task and the environment, not by the brain reproduction methods.

==> individual.tex <==
\begin{minipage}[c]{0.99\textwidth} %## ROW 1
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[BabyA]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_babya.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[BabyB]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_babyb.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[Blokky]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_blokky.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[Garrix]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_garrix.png}}
        \end{minipage}
\end{minipage}

\begin{minipage}[c]{0.99\textwidth}  %## ROW 2
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[Gecko]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_gecko.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[Insect]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_insect.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[Linkin]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_linkin.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[Longleg]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_longleg.png}}
        \end{minipage}
        \hfill
\end{minipage}

\begin{minipage}[c]{0.99\textwidth}  %## ROW 3
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[Penguin]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_penguin.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[Pentapod]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_pentapod.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[Queen]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_queen.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[Salamander]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_salamander.png}}
        \end{minipage}
\end{minipage}

\begin{minipage}[c]{0.99\textwidth}  %## ROW 4
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[Squarish]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_snake.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[Snake]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_spider.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[Spider]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_squarish.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[Stingray]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_stingray.png}}
        \end{minipage}
\end{minipage}

\begin{minipage}[c]{0.99\textwidth}  %## ROW 5
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[Tinlicker]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_tinlicker.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[Turtle]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_turtle.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[WW]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_ww.png}}
        \end{minipage}
        \hfill
        \begin{minipage}[t]{0.242\textwidth}
            \centering
            \subfloat[Zappa]{\includegraphics[width=\textwidth]{figures/images/individual/fitness_avg_max_lineplot_zappa.png}}
        \end{minipage}
\end{minipage} 
% height=2.75cm
